Improving Neural Optimal Transport via Displacement Interpolation

Optimal Transport (OT) theory investigates the cost-minimizing transport map that moves a source distribution to a target distribution. Recently, several approaches have emerged for learning the optimal transport map for a given cost function using neural networks. We refer to these approaches as the OT Map. OT Map provides a powerful tool for diverse machine learning tasks, such as generative modeling and unpaired image-to-image translation. However, existing methods that utilize max-min optimization often experience training instability and sensitivity to hyperparameters. In this paper, we propose a novel method to improve stability and achieve a better approximation of the OT Map by exploiting displacement interpolation, dubbed Displacement Interpolation Optimal Transport Model (DIOTM). We derive the dual formulation of displacement interpolation at specific time $t$ and prove how these dual problems are related across time. This result allows us to utilize the entire trajectory of displacement interpolation in learning the OT Map. Our method improves the training stability and achieves superior results in estimating optimal transport maps. We demonstrate that DIOTM outperforms existing OT-based models on image-to-image translation tasks.

==> reviewer1.tex <==
We sincerely thank the reviewer for carefully reading our manuscript and providing valuable feedback. We appreciate the reviewer for considering our work "well-written" and for acknowledging that "improving the stability of Optimal transport is an important problem". We hope our responses to be helpful in addressing the reviewer’s concerns. We highlighted the corresponding revisions in the manuscript in Brown.

$ $

---

**W1.**
(1)This method trains two optimal transport maps from source to target distribution and vice versa which is a bit inefficient. 

(2) Further, there are no experiments which demonstrate that the two independently trained transport maps are invertible, which they should be theoretically. How does source -> target -> source reconstruction perform on various datasets in the paper? Similarly, target -> source -> target reconstruction on images should be reported with a metric such as l2 error/reconstruction error.

**A.**
(1) As discussed in the limitation part of the Conclusion section (Lines 526-530), we agree with the reviewer that our DIOTM is less efficient than OTM due to the requirement to train two optimal transport maps. Nevertheless, **our approach is significantly more efficient than dynamical OT methods, such as DSBM.** By leveraging the displacement interpolation parametrization (Eq. 17), our model eliminates the need for intermediate time simulations and offers efficient generation with only 1 NFE (Number of Function Evaluations).


**We evaluated the reconstruction error of DIOTM using its bidirectional transport maps**. As a baseline, we trained two OTM models independently in both directions, i.e., $\mu \rightarrow \nu$ and $\nu \rightarrow \mu$, and measured its reconstruction error. The results are presented below:

- Reconstruction error comparison of DIOTM and OTM

|Model|8G->G->8G|G->8G->G|25G->G->25G|G->25G->G|M->S->M|S->M->S|
|OTM|   1.06    | 0.040 |  **4.13**  |  **0.56**  | 4.01  | 1.12  | 
|DIOTM| **0.22**    | **0.015** | 12.43  |  0.68  | **1.11**  | **0.46**  |

Our DIOTM achieves better reconstruction error on four out of six experiments. Our model shows a larger reconstruction error in the 25Gaussian-to-Gaussian-to-25Gaussian case ($25G \rightarrow G \rightarrow 25G$). However, this reconstruction is meaningful when the generating distribution errors are also considered, i.e., $\overrightarrow{T_{\theta}}_{\#} \mu \approx \nu$ and $\overleftarrow{T_{\theta}}_{\#} \nu \approx \mu$ (Table 1). We interpret this result as being due to the larger distribution error of OTM in the $G \rightarrow 25G$ case.

$ $

---

**W2.**
Qualitative Results: The paper should Include qualitative comparison with other methods on Image-to-Image translation baseline. FID doesn’t necessarily capture lot of semantic and perceptual information of images. A better comparison would be side-by-side comparison of images obtained from DIOTM and previous OT benchmarks.

**A.**
We included **additional qualitative comparisons of translated samples between OTM and DIOTM** in Fig 12 (Male $\rightarrow$ Female 128x128) and Fig 13 (Wiid $\rightarrow$ Cat 64x64) in the Appendix. These examples demonstrate that OTM often fails to transform target semantics correctly, e.g. resulting in Male $\rightarrow$ Male in $\lambda=50$. Furthermore, we evaluated the LPIPS score ($\downarrow)$ to quantitatively evaluate how well the generator preserves the content. The results are presented in Table 4 in the Appendix. Our model exhibits comparable LPIPS scores to the baselines.

$ $

---

**W3.**
Quantitative results: Table 2 compares DIOTM with existing neural optimal transport models. For the sake of completeness, the paper should include another table that includes other state-of-the-art methods (e.g. GANs[1], flows as well as diffusion-based methods (e.g. Wang et al. [2]) for image-to-image translation task so that reader gets an overall picture of the landscape and the gap of DIOTM from SOTA method. I would like to reiterate that it is completely alright if DIOTM is not SOTA overall, compared to other methods for I2I task, but such a table should be included, as it is a standard practice.

**A.**
In this work, our scope was to compare with OT map approaches for unpaired image-to-image translation tasks. However, **we respectfully believe that these two works are supervised approaches, and therefore not directly comparable to our unsupervised model**. Specifically, [1] employs a conditional GAN and [2] utilizes large-scale pretraining with a diffusion decoder, using the paired data. As our model is designed for unpaired image-to-image translation tasks, these methods are not appropriate for direct comparison.

$ $

---

**W4.**
Implementation details: The paper is missing some of the implementation details, specifically architecture details of networks for image-to-image translation task. Further, the number of images used to calculate FID is unclear.

**A.**
As detailed in Appendix B.2, we utilized the NCSN++ [1] as the backbone network. Note that all methods (DSBM, ASBM, OTM, and Ours) in the Image-to-Image translation tasks (Table 2) used the same backbone network. Also, regarding the FID computation, we followed the evaluation scheme of [1] for the Wild→Cat experiments and [2] for the CelebA experiments for a fair comparison. Specifically, in the Wild→Cat experiments, we generated ten samples for each source test image. Since the source test dataset consists of approximately 500 samples, we generated 5000 generated samples. Then, we computed the FID score with the training target dataset, which also contains 5000 samples. Also, in the CelebA experiment, we computed the FID score using the test target dataset, which includes 12247 samples. We generated the same 12247 samples and compared them with the test target dataset. We revised this part in the Appendix B.2 for better clarity.

[1] De Bortoli, Valentin, et al. "Schr\" odinger Bridge Flow for Unpaired Data Translation." NeurIPS 2024.

[2] Gushchin, Nikita, et al. "Adversarial Schr\" odinger Bridge Matching." NeurIPS 2024.

$ $

---

**W5.**
The largest image resolution considered in this work is 128X128 which is not very large. In order to reliably evaluate scalability, larger resolutions such as 256X256 or 512X512 should be considered. See Isola et al. [1] for a list of potential datasets for image-to-image translation tasks on larger resolution.

**A.**
Due to computational resource constraints, we were unable to conduct experiments on larger resolutions such as 256X256 or 512X512. However, considering that existing approaches in the OT literature usually evaluate their methods on resolutions comparable to or lower than 128x128 [1,2,3], 
we believe that using 128x128 resolution images can also be considered a high-dimensional experiment in the OT literature.


[1] Fan, Jiaojiao, et al. "Scalable computation of monge maps with general costs." arXiv preprint arXiv:2106.03812 4 (2021).

[2] Rout, Litu, Alexander Korotin, and Evgeny Burnaev. "Generative modeling with optimal transport maps." ICLR 2022.

[3] Gushchin, Nikita, et al. "Adversarial Schr\" odinger Bridge Matching." NeurIPS 2024.

$ $

---

**Q1.**
Training stability: Can we have multiple curves to understand how frequently the training diverges for OTM? Also, how sensitive is training of OTM to various hyperparameters?

**A.**
As shown in Fig. 4, the perfomance of OTM is highly sensitive to the regularization hyperparameter $\lambda$. In contrast, our model demonstrates robust performance to $\lambda$. 

$ $

---

**Q2.**
What are some practical constraints on the source and target distributions when trying to learn an OT map with DIOTM? Can it learn OT map in the cases where the distance between the source and target distribution might be large? For instance, prior works in this space consider more complex datasets/tasks for image-to-image translation such as mask-to-image synthesis (COCO / ADE-20K), sketch-to-image synthesis, day-to-night, summer-to-winter, colorization etc.

**A.**
We appreciate the reviewer for the thoughtful comment. The primary limitation of DIOTM for more complex tasks is that **our model assumes a quadratic cost function** $c(x,y) = \alpha \| x - y \|^{2}$. This is because the equivalence between displacement interpolation and dynamic optimal transport (Eq. 7) does not hold for general cost functions. As a result, DIOTM is not applicable to tasks where the pixel-wise quadratic cost is inappropriate. In this work, we focused on improving the stability of neural optimal transport for relatively low-resolution data. However, we believe generalizing neural optimal transport approaches to more challenging high-resolution data would be an important direction for future research.

$ $

---

**Q3.**
The results of Figure 11 seem much more suboptimal than other cases (with multiple faces) etc. What could be the reason for more failures for this pair of distribution? 

**A.**
We believe that this result happens because of \textbf{the characteristics of the Wild and Cat distributions}. In Wild images, black animals are relatively rare, except for tigers with black stripes (Fig 10, Left).  Consequently, black cats are usually translated into the tiger with black stripes (Fig 11). However, this translation incurs a relatively high cost, compared to the Male $\leftrightarrow$ Female case. We think that these unbalanced source and target distributions make image-to-image translation via the Optimal transport map more challenging in the Wild $\leftrightarrow$ Cat datasets.

$ $

---

**Minor:**
- Line 243: typo - parametrization
- Line 253, 256, 258: Consider using different parameter notation e.g. $\overrightarrow{T}_\theta$ and $\overleftarrow{T}_{\Tilde{\theta}}$ for the two transport maps, as these are parametrized with two different networks with different parameters. This would make it clear that these two networks are trained separately, as opposed to using a shared network.
- Repeated citation for Diffusion Schrodinger bridge matching paper.

**A.**
Thank you for the careful advice. We corrected the manuscript accordingly.
